Code-Optimise: Self-Generated Preference Data for Correctness and Efficiency

Code Language Models have been trained to generate accurate solutions, typically with no regard for runtime. On the other hand, previous works that explored execution optimisation have observed corresponding drops in functional correctness. To that end, we introduce Code-Optimise, a framework that incorporates both correctness (passed, failed) and runtime (quick, slow) as learning signals via self-generated preference data. Our framework is both lightweight and robust as it dynamically selects solutions to reduce overfitting while avoiding a reliance on larger models for learning signals. Code-Optimise achieves significant improvements in pass@k while decreasing the competitive baseline runtimes by an additional 6% for in-domain data and up to 3% for out-of-domain data. As a by-product, the average length of the generated solutions is reduced by up to 48% on MBPP and 23% on HumanEval, resulting in faster and cheaper inference. The generated data and codebase is open-sourced at https://github.com/huawei-noah/HEBO/tree/Code_Optimise.

==> comments.tex <==

% THIS FILE IS ONLY FOR THE CHECKLIST COMMENT/CHAT

% THE IDEA IS TO LIST EVERY POINT OF DISPUTE
% THEN ADD YOUR THOUGHTS RE: HOW TO ADDRESS EACH

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Points of Dispute

- Contribution is marginal (incremental) as other papers have shown that self-instruct can improve functional correctness.

    % OK, Leo will tackle this section
    1. Assumption and objective could be better clarified. During the idea formulation, we realised that there does not exists preference data for code, only instruction data. Additionally, the ideal preference data is locked away both technically and legally behind websites such as LeetCode and HackerRank. As such, we bootstrap existing open-source CLMs for generating the preference data using only a small set of prompts and unit tests. Clarifying this problem setup (key challenges and solutions) will better show the practical use case of our work.

    2. Reduce the emphasis on beating SFT. Instead, we should emphasise how we explore the best way to exploit the newly created code preference data, in which we found that DPO is much better than simple SFT, particularly in combination with Dynamic Solution Selection. Also, address the complaint that DPO seems weak on OOD settings. Check that the explanation for poor SFT performance is clear.   

- Code length is a confounding metric as shorter code does not imply faster code.

    % Leo as well
    1. Definition of efficiency can be better clarified. In particular, efficiency can be split into code efficiency (lower complexity) and output efficiency (lower cost). State that two metrics are being measured separately as reviewers seem to think that we associate shorter length with faster code.

    % Milan, this will take a bit of effort!
    2. Add qualitative examples. Better visualise the changes across all methods. Yeah, could truncate the y-axis to enhance differences. Does the final model generate diverse solutions? Any way to automatically assess that? One person 'complained'. Actually, more people want qualitative comparisons. Yet more queries for qualitative examples, this is a recurring theme.

    3. I would also propose to remove (some/all?) tables from the appendix, not sure it's really adding anything? Keep the appendix clean and relevant? Also, let's emphasise the difficulty of maintaining correctness while improving efficiency.

- More baseline(s), experiment(s) and dataset(s):

    % Makis can draft his 'reviewer response' for each bullet point? Perhaps we can add our thoughts, too
    1. Additional code datasets (CodeContest or PIE) and comparisons to (Shypula et al. 2023). Explain why we cannot use (Shypula et al 2023) as a baseline? Perhaps emphasise (multiple times) that the 'raw' LMs are a suitable baseline. Explain better that in their paper, achieving better runtimes has a big cost. Why do the reviewers not realise that? Then they tell us that our gains are small? :?

    % Makis: Response draft
    We should point out that our work and Shypula et al. 2023 share similar objectives but differ on the tasks; we aim to train LLMs to produce more efficient solutions given a definition prompt while Shypula et al. 2023 adapt LLMs to edit an existing piece of code to make it more efficient. As such, we cannot use the same data that Shypula et al. 2023 gathered for their task. Instead we expose the model under data sampled from its own distribution and automatically annotated with performance signal. Please also note that Shypula et al. 2023 consistently show that their speedup edits cause some programs to lose their functionality while our method and data improves both runtimes and functional accuracy.

    2. Explain why HumanEval and MBPP can be used to assess optimisation, somebody referenced (Shypula et al 2023) again :/ Why couldn't these datasets be used to evaluate runtime? Also, better emphasise that previous RL stuff DID NOT target efficiency.

    3. More experiments wanted e.g. what happens if we optimise for length, will efficiency improve? Maybe, no time though :/ Another one asked: What is we ditch the SELF in optimise and get data from other models? We had this in mind as 'distillation' and 'inverse distillation' :-o but never got to it. I think explaining that not being dependent on other LMs can be a nice advantage. I would add that 'distilled SFT' has already been done e.g. Zephyr and dozens of other papers that just grab data from ChatGPT ... lazy. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Reviewer NSxD

- What is the key challenges and how the proposed approach uniquely tackles them distinct from existing approaches? Currently, this work looks a bit incremental (self-instruct + DPO).

- (Figure 5) DPO does not seem to be effective or even bad in reducing runtimes in OOD setting. How should we overcome this?

- (Figure 6) Using code length as efficiency metric might not be a reasonable assumption, as a short program can be inefficient than a longer one. Why should we use this metric?

Reviewer M89F

- Is there any baseline method should be considered for code-optimise other than base model? In the reference (Shypulaet al. 2023), they also propose many approaches to improve performance of code and some does not depend on proprietary LLMs.

- In figure3, median runtime is showing code-optimise works both in runtime and generation length. But how much diverse are those generated code?

- In figure2, there are an obvious decrease for SFT24, SFT100 in pass@100, is this normal or any explanation?

- In figure6, the code genrated has less length for DPO. But was length a considered object when fine tune? Is there any explanation? If I say that we use LLM to optimize for short code generation, will runtime performance be improved?

- In general, is there any specific case been discussed why there is performance improvement? Code quality, Complexity optimization？

Reviewer mEn9

- The runtime speedup improvement of generated code is very small. It is hard to tell how effective the proposed method is. Since the LLMs are finetuned with the training data of MBPP, it is not really surprising that pass@k improves. Besides, the performance on HumanEval is not very good.

- The use of code length as a metric for code runtime performance is problematic. Longer code doesn't mean it's slower. A short piece of code like a lambda expression and a for loop with expensive operations in the loop can still be very slow.

- There is no real comparison baseline in the evaluation. The authors should compare their approach with the SOTA LLM-based code optimization method by Shypula et al. to demonstrate that the proposed method is indeed useful.

- The programming tasks in HumanEval and MBPP are not specifically designed for code optimization. Thus, it is hard to tell how well the proposed method is on tasks where code optimization is indeed needed and beneficial. The authors should evaluate their method on code optimization benchmarks like PIE.

- No dataset or code is made available.

Reviewer FqYX

- Contribution seems rather marginal and is not clear. Is the goal of this paper to show DPO is superior to SFT?

- Qualitative examples and analyses needed.

- To fully support the claim of encouraging the models to write more efficient code, a more challenging code generation benchmark such as CodeContests should be considered.

- What happens if we collect data using models other than the model of interest? For example, we can use chatgpt generated data to finetune StarCoder 1B. Would the proposed method still be effective, when the data come from stronger models? (1-2) Can we do better by mixing data generated from different models to construct the train set? (1-3) I think the setting of using self-generated data to finetune a model makes sense only if it belongs to one of the strongest models available at that time, thus there are no other models that can provide it with supervisory signals. Please justify the choice of using smaller models to "avoid reliance on proprietary APIs to make" your "methodology as self-contained as possible."

- When filtering data for SFT\_25 model, did you select top 25\% performing solutions for each problem or among all solutions? If the latter was the case, it could lead to problems like data imbalance, etc.

- What do you want to argue? Which one among DPO\_QvS, DPO\_PvF and DPO\_All is the best? Does the best one dominate the others in terms of execution time and correctness? Why or why not?
How does the finetuned model generate solutions that finishes execution faster? Does it learn to avoid solutions when is possible? Does it learn to use list comprehension rather than iterating over explicit loops to repeatedly append items? ... Providing some insights regarding the built train set or the finally generated samples, preferably with actual examples would be great. (4-2) Can we manually add test cases targeting large input sizes to reliably validate that the proposed method allows for generation of more efficiently implemented code?

- In the abstract the authors wrote: "However, previous work has focused on improving either functional correctness or efficiency, usually at the expense of the other." How does pursuing functional correctness harm efficiency?

Reviewer cq1E

- The paper is not particularly novel. Reinforcement learning with execution feedback for code LMs is well known and has been studied in [1][2][3]. The main differences of the current work are (1) using DPO as an alternative for RL/PPO, (2) additionally considering the runtime efficiency in feedback.

- The improvement on runtime efficiency does not generalize to a different dataset (HumanEval). For the in-domain scenario (MBPP), the improvement is somewhat small, and may be worth a statistical test for significance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Metareview:
This work presents an automatic code data augmentation method and introduces a quality control stage by running code in a code interpreter. As a result, the code data will be labeled as pass/failed and fast/slow. The authors also explore the DPO training with those labeled code data, such as guiding LLM to write time-efficient code.

Summary Of Reasons To Publish:
Introducing a code interpreter to assess the data quality and runtime behavior is well-motivated and straightforward.

The idea is easy to understand and follow.

Summary Of Suggested Revisions:
Although this work reports extensive experiment results, the comparison with existing methods is insufficient, and the results don't provide much insight.

The contribution of this work is somehow insufficient to be a long top-conference paper. Maybe reorganzing this work as a short paper is better.

Overall Assessment: 3 = There are major points that may be revised

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

RESPONSE TO REVIEWERS

Q: Contribution is marginal (incremental).
A: The paper objectives, key challenges and solutions have now been clarified. The paper has undergone extensive rewriting to address this comment and to convey the significance and suitability of our work as a long ACL paper. Some contributions were not clearly articulated giving the 'incremental' impression, this has been rectified at the end of Introduction. We substantially improved the clarity of figures as well as captions and labels to make it easier to appreciate the experiments. The dataset and code will be provided as stated in the abstract.

Q: Comparison with existing methods is insufficient and the results don't provide much insight.
A: We have reorganised the paper to make more space for this comment (Line 376, Code Efficiency Optimisation). It has been clarified why the proposed comparison with (Shypula et al 2023) or previous work in RL is not appropriate as they differ on the type of tasks (code repair versus code generation), dataset (PIE only contains functional/inefficient programs), evaluation (non-standard metrics used like best@k) and objectives (efficiency-only optimisation versus correctness and efficiency). The cited works are related but they are not suitable for direct comparison and we hope our extensive rewrites sufficiently convey this justification.

Q: Lack of qualitative analysis and examples.
A: We have added three detailed qualitative examples (two one-page figures moved to the Appendix). A new section in results now outlines the conclusions from our manual evaluation offering excellent insights into the changes induced by Code-Optimise.

Q: Code length is a confounding metric as shorter code does not imply faster code.
A: The definition of efficiency has been extensively clarified. Efficiency has been split into runtime (lower complexity) and code length (lower inference cost). Now the two metrics are being treated and reported separately.

Q: Various shorter, specific comments on methodology and/or results.
A: We also addressed specific shorter questions and smaller concerns reviewers listed in their notes for more clarity. If some suggestions could not be practically included e.g. additional experiments, we tried our best to explain why those could not be accommodated.
